Exoshuffle: An Extensible Shuffle Architecture

Shuffle is one of the most expensive communication primitives in distributed data processing and is difficult to scale. Prior work addresses the scalability challenges of shuffle by building monolithic shuffle systems. These systems are costly to develop, and they are tightly integrated with batch processing frameworks that offer only high-level APIs such as SQL. New applications, such as ML training, require more flexibility and finer-grained interoperability with shuffle. They are often unable to leverage existing shuffle optimizations. We propose an extensible shuffle architecture. We present Exoshuffle, a library for distributed shuffle that offers competitive performance and scalability as well as greater flexibility than monolithic shuffle systems. We design an architecture that decouples the shuffle control plane from the data plane without sacrificing performance. We build Exoshuffle on Ray, a distributed futures system for data and ML applications, and demonstrate that we can: (1) rewrite previous shuffle optimizations as application-level libraries with an order of magnitude less code, (2) achieve shuffle performance and scalability competitive with monolithic shuffle systems, and break the CloudSort record as the world's most cost-efficient sorting system, and (3) enable new applications such as ML training to easily leverage scalable shuffle.

==> background-2.tex <==
\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=.6\linewidth,trim=0cm 3.5cm 18cm 2.5cm, clip]{figures/shuffle-dags.pdf}
    \subcaption{``Simple'' shuffle~\cite{mapreduce,hadoop}}
    \label{fig:shuffle-dags:naive}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=.6\linewidth,trim=8cm 3.5cm 10cm 2.5cm, clip]{figures/shuffle-dags.pdf}
    \subcaption{Pre-shuffle merge~\cite{riffle}}
    \label{fig:shuffle-dags:riffle}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=.6\linewidth,trim=17cm 3.5cm 1cm 2.5cm, clip]{figures/shuffle-dags.pdf}
    \subcaption{Push-based shuffle~\cite{magnet,cosco,NADSort}}
    \label{fig:shuffle-dags:magnet}
  \end{subfigure}
  \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=.75\linewidth,trim=8cm 2.5cm 8cm 2.5cm, clip]{figures/shuffle-dag-pipeline.pdf}
    \subcaption{Pipelining shuffle~\cite{mapreduceonline}}
    \label{fig:shuffle-dags:pipeline}
  \end{subfigure}
  \caption{Shuffle algorithms in previous monolithic systems. \sys uses distributed futures to execute these as DAGs.}
  \label{fig:shuffle-dags}
\end{figure*}
\section{Background}
\label{sec:background}

Why is large-scale shuffle a challenging operation?
In a MapReduce operation with $M$ map tasks and $R$ reduce tasks, shuffle creates $M\times R$ intermediate blocks.
For example, a 100\,TB dataset with 2\,GB partitions would result in 250 million blocks of 40\,KB each.
Each of these must be moved across memory, disk, and network at least once.
This creates two challenges: (1) I/O efficiency as the number of mappers and reducers increases and the block size decreases, and (2) fault tolerance as the size of the cluster and therefore the chance of a node failure increases.
We discuss these common challenges in previous shuffle systems to identify the common solution requirements.
These will motivate our use of distributed futures in \Cref{sec:shuffle}.

We first consider I/O efficiency.
When the total data size exceeds total memory, data must be spilled to persistent storage.
Current data warehouses primarily use hard disk drives (HDD), due to cost-effectiveness and longevity compared to SSDs~\cite{ssd-design}.
HDDs can provide at most hundreds of I/O operations per second (IOPS), and have much lower random I/O throughput than sequential I/O.
In a naively executed large-scale shuffle~(\cref{fig:shuffle-dags:naive}), the small intermediate blocks create a disk bottleneck.
Previous optimizations on reducing I/O overhead fall under two general catagories:
(1) reducing the number of small and random I/O accesses by adding \emph{coordination} between mappers and reducers to merge intermediate blocks into larger ones~\cite{riffle,cosco}, and (2) optimizing \emph{block management} to overlap I/O with execution, i.e. pipelining~\cite{magnet,sparkshufflemagic}.

\paragraph{\bf Distributed coordination.}
First, many shuffle systems merge intermediate shuffle blocks into larger ones to increase disk I/O efficiency~\cite{sparkshufflemagic,magnet,riffle,cosco}.
For example, Riffle~\cite{riffle} merges map outputs that reside on the same mapper node, reducing the total number of blocks by a constant factor~(\cref{fig:shuffle-dags:riffle}).
Magnet~\cite{magnet} and Cosco~\cite{cosco} merge map outputs from different mapper nodes before the final reduce stage~(\cref{fig:shuffle-dags:magnet}).
All of these systems require additional \emph{external shuffle services} and protocols to coordinate between the mappers, intermediate mergers, and reducers~\cite{sparkpetabyteblog,riffle,magnet,cosco}.

Meanwhile, with distributed futures, we can offload coordination between executors to the underlying system.
The shuffle application uses distributed futures to express the optimizations studied in previous shuffle systems as task DAGs.
For example, it can express \Cref{fig:shuffle-dags:riffle,fig:shuffle-dags:magnet} by passing the distributed futures returned by a map task to an intermediate merge task, then passing those outputs to a final reduce task~(\cref{sec:shuffle}).
The system is then responsible for fulfilling the dependencies in the resulting DAG.


\paragraph{\bf Pipelining execution.}
Achieving high performance in shuffle also requires overlapping network I/O, disk I/O, and execution.
Traditional shuffle is pull-based~(\cref{fig:shuffle-dags:naive}): reduce tasks only pull the shuffle blocks from the map tasks once the map stage is complete, which limits pipelining~\cite{mapreduceonline}.

A common solution for pipelining execution and disk I/O is to increase task parallelism, allowing one task to write to disk while another executes~\cite{magnet}.
To pipeline network I/O, some systems use push-based shuffle~\cite{NADSort,magnet,cosco,ishuffle}.
In this scheme, mappers push their outputs immediately to the reducers, where they can be partially merged on disk before the final reduce stage~(\cref{fig:shuffle-dags:magnet}).
Such pipelining is also valuable for overlapping shuffle tasks with other workloads~\cite{mapreduceonline}, as shown in \Cref{fig:shuffle-dags:pipeline}.

All of these solutions can be considered different optimizations within block management.
Thus, rather than re-implement them manually with each new shuffle system, we propose using distributed futures as a common interface for block management.
Each distributed future represents a block, whose value may be pending computation, stored in memory, stored on disk, in the network, or any combination of the above.
These decisions are left to the system, allowing it to pipeline block movement across resources within a shuffle job~(\cref{fig:shuffle-dags:pipeline}).
Furthermore, the use of distributed futures as a common interface enables interoperability with any \emph{other} job that can consume a distributed future~(\cref{fig:shuffle-dags:pipeline}).

\paragraph{\bf Handling executor and network failures.}
Shuffle is an all-to-all communication, making connection and transfer failures between mappers and reducers inevitable as the cluster size grows.
Moreover, if a map executor process dies, e.g., due to memory pressure, the reduce tasks will not be able to fetch their inputs, even if the results are still on the mapper's disk.
In addition to minimizing interruptions from failure, the shuffle system must also guarantee consistency, i.e., that each record in the input appears exactly once in the output.

Current state-of-the-art shuffle systems run an external shuffle service to minimize interruptions upon map executor failures~\cite{sparkpetabyteblog,magnet}.
The external service manages on-disk block metadata, decoupling the lifetime of executor processes from the lifetime of shuffle blocks.
Shuffle systems additionally use custom techniques to ensure exactly-once semantics.
Magnet, for example, uses best-effort semantics to merge intermediate outputs, then falls back to reducing map outputs directly upon failure~\cite{magnet}.
Cosco uses a combination of replication and deduplication~\cite{cosco}.

We show how a distributed futures system can provide these properties. % that guarantees that any distributed future referenced by the application can be eventually resolved to its value, even in the presence of failures.
First, similar to an external shuffle service, a distributed object store decouples the lifetimes of intermediate blocks and individual executors.
Second, in the case of an object store failure, the system can minimize interruptions by using \emph{lineage reconstruction}, i.e. re-executing the DAG that created the lost object.
These techniques are well-studied in previous work on DAG-based execution frameworks~\cite{spark-rdd,ownership,mapreduce,isard2007dryad}.
Lineage reconstruction makes it simple to guarantee exactly-once semantics because objects are immutable and task dependencies are fixed.
As long as the application can make each task deterministic and side-effect-free, each input record will appear in the output exactly once.
Thus, we show that with generic per-block fault tolerance, we can achieve the same degree of fault tolerance as previous systems with manual recovery techniques.


==> intro-2.tex <==
\section{Introduction}
\label{sec:intro}

Shuffle is a key primitive in many data processing applications.
It is the foundation of the MapReduce model~\cite{mapreduce} and large-scale data processing applications such as distributed sort.
Large-scale shuffle operations are also difficult to execute efficiently and reliably because they entail \emph{all-to-all} communication to transfer data from the mappers to the reducers~\cite{riffle}.

The key challenge in large-scale shuffle is efficiently moving the large number of very small intermediate blocks from each mapper to each reducer.
For example, LinkedIn reports that its Spark clusters shuffle billions of blocks daily, with an average block size of only tens of KBs~\cite{magnet}.
Scaling shuffle thus requires both high I/O efficiency to move blocks across memory, disk, and network, as well as reliability in the presence of node or network failures.

The difficulty of this problem has inspired a myriad of shuffle implementations, each of which is essentially built from scratch using low-level primitives like RPC to coordinate and execute block transfers.
These have led to breakthroughs in shuffle performance and reliability.
However, implementing shuffle as a monolithic system comes with a cost: \emph{flexibility}.

First, designing and implementing a shuffle system is a significant developer effort, often impeding innovation.
Magnet, for example, achieves 30\% end-to-end performance improvement by having mappers push intermediate blocks directly to reducers (``push-based shuffle'')~\cite{magnet}.
However, Magnet took 14 months between publication and open-source release in the Spark project~\cite{spark-3-2-0} because it requires a complete rewrite of the shuffle system.

Second, while shuffle systems are of course highly optimized for shuffle operations, they are not flexible enough to interoperate with other applications.
The semantics offered by existing shuffle system are \emph{synchronous}: the shuffle results can only be used once all reduce tasks complete.
This is a problem for applications that require fine-grained pipelining, where downstream tasks consume shuffle outputs as they become ready, rather than wait for the entire shuffle to complete.
For example, supporting online aggregation~\cite{online-aggregation} by streaming results to the user requires extensive modifications to existing MapReduce systems~\cite{mapreduceonline,g-ola}.
As another example, distributed model training often requires shuffling the entire dataset between epochs to improve training quality~\cite{randomreshuffling}, and the training workers rely on fine-grained pipelining of shuffle outputs into model training inputs to reduce latency.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=0.5cm 4.5cm 15.5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{Monolithic shuffle systems.}
    \label{fig:shuffle-arch:monolithic}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=11cm 4.5cm 5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{\sys.}
    \label{fig:shuffle-arch:exoshuffle}
  \end{subfigure}
  \label{fig:shuffle-arch}
  \caption{\sys enables application-level (red boxes) shuffle implementations that are both high-performance and able to tightly integrate with other applications.
  }
\end{figure}

We argue that these flexibility problems stem from the design of shuffle as a monolithic system~(\cref{fig:shuffle-arch:monolithic}).
Current shuffle systems manually implement all aspects of block management.
Thus, optimizations such as push-based shuffle require rewriting a large fraction of the shuffle system~\cite{magnet}.
Meanwhile, supporting fine-grained pipelining would also require extensive changes in both the semantics and implementation of the shuffle system~\cite{mapreduceonline}.

The popular wisdom is that specialized systems are necessary for shuffle performance because of a fundamental tradeoff between performance and flexibility.
We show that this is not the case:
shuffle can be implemented at the application level, with high performance and reliability, on a generic distributed computing system~(\cref{fig:shuffle-arch:exoshuffle}).
In this paper, we show that with a task-based distributed futures system, it is possible to:
(1) express past optimizations, such as push-based shuffle, in a few hundred lines of application-level Python code, and
(2) support streaming shuffle applications, such as for distributed training, by expressing fine-grained pipelining in application code.

In order to easily implement new optimizations and achieve application interoperability, shuffle needs to be decoupled from low-level system components and be implemented at the application level.
This requires separating the control path, where the driver coordinates the transfer of shuffle blocks, from the data path, where the blocks are transferred between worker nodes.
This is traditionally difficult to achieve since in vanilla RPC, data is passed by value with the message.
What we desire is an abstraction that enables passing object references to remote tasks, such that physical data movement can be decoupled from control messages.

We propose using the \emph{distributed futures} abstraction~\cite{ciel,ownership,hotos-rpc} to express shuffle at the application level.
A distributed future is a first-class reference to a globally shared and immutable address space.
To create a distributed future, the application invokes a remote function, or \emph{task}.
For example, a mapper could be expressed as a task that returns a list of distributed futures, each representing one intermediate block.
Before the value is computed, the application may pass the distributed future as an argument to a subsequent task.
The system is then responsible for resolving the task arguments to their physical values once computed, and executing the dependent task.
The distributed futures abstraction makes it simple to express various shuffle algorithms (\cref{fig:shuffle-dags}) as application-level programs (\cref{lst:simple-shuffle,lst:two-stage-shuffle}).

However, while distributed futures make it simple to express shuffle, it is not yet clear whether these implementations can achieve high performance.
Unlike a specialized shuffle system, which has a notion of a map and a reduce stage and can optimize transfer of intermediate blocks accordingly, a distributed futures system is generic and must execute work at the unit of a function call.
Indeed, while the system Dask currently uses distributed futures to implement sort, the Dask authors recently prototyped a shuffle implementation that in effect bypasses the Dask distributed futures backend because of performance limitations~\cite{dask-better-shuffling}.

Why is it challenging for shuffle systems to achieve high performance?
First, the shuffle system must manage \emph{distributed coordination} between the mappers and reducers, to ensure that each intermediate block is moved to the appropriate reducer.
Second, the shuffle system must manage the \emph{efficient transfer of intermediate blocks} across memory, disk, and network.
Finally, the shuffle system must ensure \emph{fault tolerance}, i.e. each record in the input should appear in the output exactly once and failures should impede progress as little as possible.

We identify the components of a distributed futures system implementation that are necessary for shuffle performance and reliability.
First, for coordination, we use a distributed object store that acts as an intermediary between the map and reduce tasks: map tasks store their outputs in the object store and reduce tasks retrieve their arguments from the object store.
Second, for block management, the system orchestrates transparent data movement between the object store and local disk and across the network, to fulfill the task dependencies specified by the application.
The system also implements timely garbage collection to ensure object store availability.
Finally, for fault tolerance, the system uses lineage reconstruction to ensure that each object is reachable in the presence of failures.


Thus, we present \sys, a flexible shuffle system that recasts past work in shuffle systems as distributed futures applications.
We built \sys on Ray, a task-based distributed futures system for Python~\cite{ray,ownership}.
To meet the demands of large-scale shuffle, we extended Ray with automatic memory management of the object store and high-throughput spilling to disk~(\cref{sec:arch}).
We show that the \sys implementations of previous shuffle strategies match the performance characteristics of their monolithic counterparts.
We also ran a 100\,TB TeraSort benchmark on a cluster of 100 HDD nodes and found that \sys outperformed Spark by $1.8\times$.
Finally, we show that \sys can easily integrate with applications such as distributed training through fine-grained pipelining, reducing the latency to the first result by 70\%.
In summary, our contributions are:
\begin{itemize}
    \item Identifying the common components of shuffle systems that can be factored out into distributed futures~(\cref{sec:background}).
    \item Showing how optimizations from previous monolithic shuffle systems can be expressed as distributed futures programs~(\cref{sec:shuffle}).
    \item Designing and building a distributed futures system that can execute large-scale application-level shuffle~(\cref{sec:arch}), which outperforms Spark on a 100\,TB shuffle on 100 nodes, and can easily interoperate with other applications through fine-grained pipelining~(\cref{sec:eval}).
\end{itemize}








==> intro-3.tex <==
\section{Introduction}
\label{sec:intro}

Shuffle is a key primitive in data processing.
It is the foundation of the MapReduce model~\cite{mapreduce} and large-scale data processing applications such as distributed sort.
Large-scale shuffle operations are also difficult to execute efficiently and reliably because they entail \emph{all-to-all} communication to transfer data from the mappers to the reducers~\cite{riffle}.

The key challenge in large-scale shuffle is efficiently moving the large number of very small intermediate blocks from each mapper to each reducer.
For example, LinkedIn reports that its Spark clusters shuffle billions of blocks daily, with an average block size of only tens of KBs~\cite{magnet}.
Scaling shuffle thus requires both high I/O efficiency to move blocks across memory, disk, and network, as well as reliability in the presence of node or network failures.

The difficulty of this problem has inspired a myriad of shuffle implementations, each of which is essentially built from scratch using low-level primitives like RPC to coordinate and execute block transfers.
These have led to breakthroughs in shuffle performance and reliability.
However, implementing shuffle as a monolithic system comes with a cost: \emph{flexibility}.

First, designing and implementing a shuffle system is a significant developer effort, often impeding innovation.
Magnet, for example, achieves 30\% end-to-end performance improvement by having mappers push intermediate blocks directly to reducers (``push-based shuffle'')~\cite{magnet}.
However, Magnet took 19 months between publication and open-source release in the Spark project~\cite{spark-3-2-0} because it required a complete rewrite of the shuffle system.

Second, while shuffle systems are of course highly optimized for shuffle operations, they are not flexible enough to interoperate with other applications.
The semantics offered by existing shuffle systems are \emph{synchronous}: the shuffle results can only be used once all reduce tasks complete.
This is a problem for applications that require fine-grained pipelining, where downstream tasks consume shuffle outputs as they become ready instead of waiting for the entire shuffle to complete.
For example, supporting online aggregation~\cite{online-aggregation} by streaming results to the user requires extensive modifications to existing MapReduce systems~\cite{mapreduceonline,g-ola}.
As another example, distributed model training often requires repeatedly shuffling the training dataset between epochs to improve learning quality~\cite{randomreshuffling}.
Fine-grained pipelining of the shuffle and training tasks is necessary for overall throughput.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=0.5cm 4.5cm 15.5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{Monolithic shuffle systems.}
    \label{fig:shuffle-arch:monolithic}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=11cm 4.5cm 5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{\sys.}
    \label{fig:shuffle-arch:exoshuffle}
  \end{subfigure}
  \label{fig:shuffle-arch}
  \caption{\sys enables application-level (red boxes) shuffle implementations that are both high-performance and able to tightly integrate with other applications.
  }
\end{figure}

We argue that these flexibility problems stem from the design of shuffle as a monolithic system~(\cref{fig:shuffle-arch:monolithic}).
Current shuffle systems build on messaging primitives like RPC to implement both the control plane, which decides which blocks should be transferred to which nodes, and the data plane, which implements the physical block transfer.
The result is a tight coupling between the control and data planes.
Thus, although many previous optimizations such as push-based shuffle and fine-grained pipelining mainly involve control plane decisions, their implementations require rewriting a large fraction of the shuffle system~\cite{magnet,mapreduceonline}.

The popular wisdom is that this design approach is necessary for achieving shuffle performance.
We show that this is not the case:
by decoupling the shuffle control plane from the shuffle data plane, we can implement shuffle at the application level and achieve flexibility without loss of performance or reliability~(\cref{fig:shuffle-arch:exoshuffle}).
In this paper, we show that with a generic task-based distributed futures~\cite{ciel,ownership,hotos-rpc} system, it is possible to:
(1) express past optimizations, such as push-based shuffle, in a few hundred lines of application-level Python code, and
(2) support fine-grained interoperability between shuffle and other applications such as distributed training.

In order to decouple the shuffle control and data planes, we require an abstraction that allows the application to specify where block data should be moved without having to see the physical data.
This rules out RPC as a common primitive for application-level shuffle, as RPC requires all data values to be copied between the sender and receiver.
Instead, we desire a higher-level abstraction that moves responsibility over the physical data into a common shuffle-agnostic system.

We propose using the \emph{distributed futures} abstraction~\cite{ciel,ownership,hotos-rpc} for this purpose.
A distributed future is a first-class reference to a globally shared and immutable address space.
To create a distributed future, the application invokes a remote function, or \emph{task}.
For example, a mapper could be expressed as a task that returns a list of distributed futures, each representing one intermediate block.
Before the value is computed, the application may pass the distributed future as an argument to a subsequent task.
The system is then responsible for resolving the task arguments to their physical values once computed, and executing the dependent task.
Thus, the distributed futures abstraction makes it simple to express and modify the shuffle control plane as an application-level program.

Meanwhile, the data plane, i.e. the distributed futures backend, must deliver the same performance and reliability as a monolithic shuffle system.
Unlike a specialized shuffle system, which has a notion of a map and a reduce stage and can optimize transfer of intermediate blocks accordingly, a distributed futures system is generic and must execute work at the unit of a function call.
Indeed, while the system Dask currently uses distributed futures to implement sort, the Dask authors recently prototyped a shuffle implementation that in effect bypasses their distributed futures backend because of performance limitations~\cite{dask-better-shuffling}.

To implement an efficient and generic data plane for shuffle, we must first consider what makes large-scale shuffle challenging.
First, the shuffle system must manage \emph{distributed coordination} between the mappers and reducers, to ensure that each intermediate block is moved to the appropriate reducer.
Second, the shuffle system must manage the \emph{efficient transfer of intermediate blocks} across memory, disk, and network.
Finally, the shuffle system must ensure \emph{fault tolerance}: each record in the input should appear in the output exactly once and failures should impede progress as little as possible.

Next, we identify the components of a distributed futures system implementation that are necessary for shuffle performance and reliability.
First, for coordination, we use a distributed object store that acts as an intermediary between the map and reduce tasks: map tasks store their outputs in the object store and reduce tasks retrieve their arguments from the object store.
Second, for block management, the system orchestrates transparent data movement, both between the object store and local disk and across the network, to fulfill the task dependencies specified by the application.
The system also implements timely garbage collection to ensure object store availability.
Finally, for fault tolerance, the system uses lineage reconstruction to ensure that each object is reachable in the presence of failures.


Thus, we present \sys, a flexible shuffle system that recasts past work in shuffle systems as distributed futures applications.
We built \sys on Ray, a task-based distributed futures system for Python~\cite{ray,ownership}.
To meet the demands of large-scale shuffle, we extended Ray with automatic memory management of the object store and high-throughput spilling to disk~(\cref{sec:arch}).
We show that the \sys implementations of previous shuffle strategies match the performance characteristics of their monolithic counterparts.
We also ran a 100\,TB TeraSort benchmark on a cluster of 100 HDD nodes and found that \sys outperformed Spark by $1.8\times$.
Finally, we show that \sys can easily integrate with applications such as distributed training through fine-grained pipelining, reducing the latency to the first result by 70\%.
In summary, our contributions are:
\begin{itemize}
    \item Identifying a common data plane for shuffle that can be decoupled from the control plane via distributed futures~(\cref{sec:background}).
    \item Showing how control plane optimizations from previous specialized shuffle systems can be expressed at the application level~(\cref{sec:shuffle}).
    \item Designing and building a distributed futures system~(\cref{sec:arch}) that can match Spark on a 100\,TB shuffle on 100 nodes with an application-level shuffle, and that can easily interoperate with other applications through fine-grained pipelining~(\cref{sec:eval}).
\end{itemize}








==> intro-4.tex <==
\section{Introduction}
\label{sec:intro}
\samyu{"Sounds like there are two applications, you build two shuffle libraries, you're good" but what we're really trying to say is there's a large set of diverse applications and we can solve all their problems with one API that forms a narrow waist}

\samyu{Paragraphs 3-6 are long and can be cut down; they go into a lot of detail about specific problems with shuffle, but that's not the problem we're actually solving (doesn't lead immediately to the intermediate layer thing). Maybe take topic sentences of these paragraphs and pick one example.}

\samyu{laundry list 4-ish applications that all depend on shuffle-style data movement but look like they need different things, and show we can have a unified framework for all of these.}

\samyu{shift focus to motivating narrow waist and then explain challenges and proposed solution; leave details on RPC, etc to later in the paper}

\samyu{Use "abstraction" instead of library to make it sound cooler and more general}

\samyu{"We're using distributed futures to propose a unified abstraction for a shuffle API with which a variety of shuffle algorithms can be expressed"?}

\samyu{What's the key contribution? Reusability or evolvability? Seems like it should be the common abstraction that people can reuse (say, 80\% of the impl) and then tweak for their app. Evolvability suggests that shuffle has to change over time. Idea that a single application has to redo shuffle impls for different FT, hardware needs gets lost.}

\samyu{explicitly (in the text, not just via references) talk about the example where FB reimplemented shuffle systems for same application -- 3rd par, sentence 1 is supposed to say this, but maybe it's not coming across}

\samyu{From Chris "very application-centric, doesn't talk about stuff like resource management, fairness, security and stuff that's involved in the external shuffle service"}

\samyu{Current argument comes across as "there's one best shuffle" and that changing is a consequence of changing hardware, etc., but that's not what we're trying to say}

\samyu{mentioning "narrow waist for shuffle" might help clarify}

\samyu{RPC discussion: if we're not the first to use distributed futures for this (per end of intro), do we actually need the RPC discussion or can we just push it to motivation?}

\samyu{for contribution: others have shown specific shuffle implementations on distributed futures interface, but we provide a more general framework}

\samyu{in abstract: highlight contribution of decoupling data and control plane more, maybe separate that from Ray as the implementation mechanism}

\samyu{keep the figure and the discussion around it :)}

\samyu{move systems requirements further up? i.e., distributed futures API wouldn't work for large-scale shuffle if the underlying system couldn't spill to disk}

Shuffle is a key primitive in data processing.
It is the foundation of the MapReduce model~\cite{mapreduce} and large-scale data processing applications such as distributed sort.
Large-scale shuffle operations are also difficult to execute efficiently and reliably because they entail \emph{all-to-all} communication to transfer data from the mappers to the reducers.

The key challenge in large-scale shuffle is efficiently moving the large number of very small intermediate blocks from each mapper to each reducer.
For example, LinkedIn reports that its Spark clusters shuffle billions of blocks daily, with an average block size of only tens of KBs~\cite{magnet}.
Scaling shuffle thus requires both high I/O efficiency to move blocks across memory, disk, and network, as well as reliability in the presence of node or network failures.

The difficulty of this problem has inspired a myriad of shuffle implementations that have produced breakthroughs in performance and reliability, often by optimizing for varying end application requirements such as larger data sizes or new storage hardware~\cite{XXXmanyshufflesystemshere}.
However, in practice, many applications cannot benefit from such innovations because of the difficulty of \emph{evolving} existing shuffle implementations.

Today's shuffle implementations are difficult to evolve because they are tightly integrated into a framework that hides the shuffle details under a higher-level abstraction such as SQL.
Thus, the best option for shuffle innovations to achieve practical impact is to integrate with such open-source frameworks as Apache Spark or Hadoop. %, so that end applications can directly benefit without having to modify their higher-level code.
Unfortunately, such integration rarely happens because it incurs a high development cost.
Magnet, for example, achieves 30\% end-to-end performance improvement by having mappers push intermediate blocks directly to reducers (``push-based shuffle'')~\cite{magnet}.
However, Magnet took 19 months between publication and open-source release in the Spark project~\cite{spark-3-2-0}, with significant changes to system internals~\cite{spark32915}.

Furthermore, while these frameworks are of course highly optimized for shuffle operations, they are not always well suited to the needs of end applications.
For example, online aggregation and continuous queries are a poor fit for MapReduce-like frameworks that require all outputs to be materialized before being consumed~\cite{mapreduceonline}.
Another recent example is data shuffling for ML pipelines.
Distributed model training often requires repeatedly shuffling the training dataset between epochs to improve learning quality~\cite{randomshuffling}.
Doing this efficiently requires \emph{fine-grained pipelining} between shuffle and training: the downstream ML trainers should consume shuffle outputs as they become ready.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=0.5cm 4.5cm 15.5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{Monolithic shuffle systems.}
    \label{fig:shuffle-arch:monolithic}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=11cm 4.5cm 5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{\sys.}
    \label{fig:shuffle-arch:exoshuffle}
  \end{subfigure}
  \label{fig:shuffle-arch}
  \caption{\sys enables application-level (red boxes) shuffle implementations that are both high-performance and able to tightly integrate with other applications.
  }
\end{figure}

Thus, to serve different application requirements, framework developers must continue to rebuild shuffle from scratch, often with significant limitations from the high development cost.
For example, distributed data loaders designed specifically for ML can pipeline shuffle with the training execution but cannot disaggregate shuffle resources or perform distributed shuffle, limiting the range of application support.

In this paper, we study the problem of building high-performance distributed shuffle in a flexible and reusable way.
Today, shuffle is built in a \emph{monolithic} manner, as an integral part of a higher-level framework or in some cases as a standalone service~(\Cref{fig:shuffle-arch:monolithic}).
The key idea behind our solution is to expose distributed shuffle as a \emph{library}~(\Cref{fig:shuffle-arch:exoshuffle}).
By doing so, we can both: (1) allow shuffle builders to easily develop and integrate new shuffle designs, and (2) allow a broader set of applications to easily leverage and choose between existing shuffle implementations.
Note that this does not require exposing shuffle to \emph{end} applications; such decisions can continue to be made by a higher-level application framework, e.g., for ML data loading.

The main challenge in providing shuffle-as-a-library is to design a suitable \emph{intermediate layer} for building different shuffle implementations.
Such a layer must be: (1) sufficiently high-level that it can abstract away common parts of different shuffle systems, such as block I/O and fault tolerance, (2) sufficiently low-level that arbitrary applications and frameworks can be built atop, and (3) high-enough performance that shuffle libraries built atop can feasibly substitute for monolithic shuffle systems.

The choice of intermediate layer in existing system architectures reveals the reasons shuffle has thus far failed to achieve flexibility.
Monolithic shuffle systems build shuffle on messaging primitives like RPC.
As a messaging abstraction, RPC is both general-purpose and high-performance, but it is too low-level to act as a useful intermediate layer for shuffle.
It requires new shuffle designs to implement entirely new protocols alongside existing ones.
Integrating push-based shuffle into Spark, for example, required 1k+ LoC for the RPC layer changes alone~\cite{}.

The key problem is that \emph{RPC tightly couples the shuffle control and data planes}.
It is used to implement both the control plane, which decides which blocks should be transferred to which nodes, and the data plane, which implements the physical block transfer between processes.
Thus, although many optimizations such as push-based shuffle and fine-grained pipelining mainly involve control plane decisions, their implementations require rewriting much of the dataplane as well~\cite{magnet,mapreduceonline}.

To decouple the shuffle control plane from the shuffle data plane, we use the \emph{distributed futures} abstraction~\cite{ciel,ownership,hotos-rpc} as an intermediate layer.
Distributed futures are an extension of RPC that adds the ability to reference a globally shared and immutable address space.
To create a distributed future, the application invokes an RPC, or a \emph{task}.
For example, a mapper could be expressed as a task that returns a list of distributed futures, each representing one intermediate block.
Before the value is computed, the application may pass the distributed future as an argument to a subsequent task.
The system is then responsible for resolving the task arguments to their physical values once computed, executing the dependent task, and garbage-collecting the arguments once all references have gone out of scope.
Thus, the distributed futures abstraction makes it simple to express and modify the shuffle control plane as an application-level library.

Meanwhile, all shuffle libraries can share a common data plane, i.e. the distributed futures backend.
The data plane must deliver the same performance and reliability as a monolithic shuffle system.
This is challenging because of the granularity of system operations: unlike a specialized shuffle system, which has a notion of a map and a reduce stage and can optimize transfer of intermediate blocks accordingly, a distributed futures system is not specific to shuffle and must treat each task and object as an independent unit.
Indeed, while the system Dask offers a distributed futures-based shuffle, the Dask authors actually recommend using a custom shuffle implementation that bypasses their distributed futures backend because of scheduler scalability limits~\cite{dask-better-shuffling}.


We identify the components of a distributed futures system implementation that are necessary for performance and reliability of shuffle-as-a-library.
First, to coordinate the shuffle between mappers and reducers, we use a shared-memory distributed object store that acts as an intermediary: map tasks store their outputs in the object store and reduce tasks retrieve their arguments from the object store.
Second, for efficiency, the system transparently overlaps task execution with block I/O across the shared-memory object store, local disk, and network.
The system also implements timely garbage collection to ensure memory availability and reduce write amplification.
Finally, for fault tolerance, the system uses lineage reconstruction to ensure that each object required by the shuffle library is still reachable in the presence of failures.


Thus, we present \sys, a flexible shuffle system.
We build \sys on Ray, a distributed futures system for Python~\cite{ray,ownership}.
To meet the demands of large-scale shuffle, we extend Ray in several ways, including high-throughput spilling to disk and pipelining between block I/O and execution~(\cref{sec:arch}).
We show that the \sys implementations of previous shuffle strategies match the performance characteristics of their monolithic counterparts.
We also run a 100\,TB TeraSort benchmark on a cluster of 100 HDD nodes and find that \sys outperforms Spark by $1.8\times$.
Finally, we show that \sys can easily integrate with applications such as distributed ML training, improving end-to-end training throughput by $2.4\times$.
Thus, although we are not the first to propose using distributed futures as an intermediate layer for shuffle\lsf{Who was the first?}, we:
\begin{itemize}
    \item Show how existing shuffle optimizations can be rewritten as libraries using an order of magnitude less code.
    \item Produce a distributed futures implementation that scales shuffle to 100\,TB or more, matching or exceeding the performance of monolithic shuffle systems.
    \item Enable a broader set of applications to easily leverage previous shuffle work.
\end{itemize}









==> intro-5.tex <==
\section{Introduction}
\label{sec:intro}

Shuffle is a key operation in distributed data processing.
It is the foundation of the MapReduce model~\cite{mapreduce} and large-scale data processing applications such as distributed sort.
Large-scale distributed shuffle is difficult to execute because it entails \emph{all-to-all} communication to transfer data from the mappers to the reducers.
This requires efficiently and reliably moving a large number of small intermediate blocks from each mapper to each reducer, across memory, disk, and network. For terabyte-scale data, this can result in millions of transfers.
Furthermore, the system must be robust to potential node failures and data skew.


Applications of shuffle span a continually evolving range of execution models~\cite{mapreduce,spark-rdd,unifying-data-loading} and requirements, including scaling data size~\cite{riffle,magnet} and adapting to new storage systems or hardware~\cite{cosco,awsglueshuffle}.
Since the introduction of MapReduce, the industry and research community has repeatedly produced new shuffle implementations in response to these requirements.
While this has collectively led to breakthroughs in shuffle performance and reliability, in practice many applications cannot benefit from such innovations because of the difficulty of evolving shuffle implementations. \samyu{TODO: define evolving}

Today's shuffle implementations are tightly integrated into frameworks that hide the shuffle details under a higher-level abstraction such as SQL~(\Cref{fig:shuffle-arch:monolithic}).
Thus, to reach end applications, shuffle builders have two options.

On one hand, they can integrate new shuffle designs into existing open-source frameworks such as Spark or Hadoop.
Unfortunately, such integration rarely happens because it incurs a high development cost.
Magnet, for example, uses push-based shuffle
to achieve 30\% end-to-end performance improvement~\cite{magnet}.
However, Magnet took 19 months between publication and open-source release in the Spark project~\cite{spark-3-2-0}, with significant changes to system internals~\cite{spark32915}.

On the other hand, developers can rebuild the entire framework from the ground up.
This is often necessary to interoperate with new application models.
For example, online aggregation requires extensive modifications to the MapReduce system to stream results to the user~\cite{mapreduceonline}.
Another example is data shuffling for ML pipelines.
Distributed model training often requires repeatedly shuffling the training dataset between epochs to improve learning quality~\cite{randomreshuffling,sgd-shuffle}, which requires \emph{fine-grained pipelining} for efficiency.
To support these applications, framework developers have turned to rebuilding shuffle from scratch, often with significant limitations to reduce the development cost.
For example, distributed ML data loaders can pipeline shuffle with the training execution but cannot disaggregate shuffle resources or perform distributed shuffle~\cite{unifying-data-loading}. %, limiting the range of application support.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=0.5cm 4.5cm 15.5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{Monolithic shuffle systems.}
    \label{fig:shuffle-arch:monolithic}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\linewidth}
    \centering
    \includegraphics[bb=0 0 720 405,width=\textwidth,trim=11cm 4.5cm 5cm 4.5cm, clip]{figures/exoshuffle.pdf}
    \subcaption{\sys.}
    \label{fig:shuffle-arch:exoshuffle}
  \end{subfigure}
  \vspace*{-1ex}
  \label{fig:shuffle-arch}
  \caption{\sys enables application-level (red boxes) shuffle implementations that are both high-performance and able to tightly integrate with other applications.
  }
\end{figure}

In this paper, our goal is to design a common intermediate layer for distributed shuffle that would enable flexible, efficient, and portable implementations.
Today, shuffle is built in a \emph{monolithic} manner, as an integral part of a higher-level framework or sometimes as a standalone service~(\cref{fig:shuffle-arch:monolithic}).
The key idea behind our solution is to expose distributed shuffle as a \emph{library}~(\cref{fig:shuffle-arch:exoshuffle}).
By doing so, we can both: (1) allow shuffle builders to easily develop and integrate new shuffle designs, and (2) allow a broader set of applications to easily leverage existing shuffle optimizations.

The main challenge in providing shuffle-as-a-library is to design a suitable abstraction for building different shuffle implementations.
Such a layer must be: (1) sufficiently high-level that it can abstract away common parts of different shuffle systems, such as block I/O and fault tolerance, (2) sufficiently low-level that arbitrary applications and frameworks can be built atop, and (3) high-enough performance that shuffle libraries built atop can practically substitute for monolithic shuffle systems.

Monolithic shuffle systems generally build shuffle on top of messaging primitives like RPC and therefore \emph{tightly couple} the shuffle control and data planes.
RPC is used to implement both the control plane, which decides which blocks should be transferred to which nodes, and the data plane, which implements the physical block transfer between processes.
Thus, although many optimizations such as push-based shuffle and fine-grained pipelining mainly involve control plane decisions, their implementations require rewriting much of the dataplane as well~\cite{magnet,mapreduceonline}.

We use \emph{distributed futures}~\cite{ciel,ownership,hotos-rpc} as an abstraction to decouple the shuffle control plane from the shuffle data plane.
Distributed futures are an extension of RPC that adds the ability to reference a globally shared and immutable object store. %\ion{We should either use "object store" or "address space" throughout the paper and intro} \ion{With distributed futures, instead of including the data arguments in the RPC call, we include the pointers (i.e., distributed futures) to the data which is already stored, or yet to be created and stored, in the shared address space.}
In contrast to RPC, for which all arguments must be copied from the caller to the executor, distributed futures allow the caller to pass arguments \emph{by pointer}; the system then implements the physical data transfer to the executor through the shared object store.
Distributed futures can also be passed before the data has been created, allowing the system to parallelize remote calls and pipeline data transfer with remote execution.
For example, a mapper can be expressed as an RPC call, i.e. a \emph{task} that returns a list of distributed futures, each representing one intermediate block.
The caller can specify the shuffle by passing one distributed future to each reduce task.

\lsf{Distributed futures itself is not enough; need a high-performance data plane}

While we are not the first to use distributed futures to execute shuffle~\cite{ciel,dask}, our contribution is in showing how this abstraction can serve as a narrow waist for arbitrary shuffle algorithms.
To do so, we study the design and implementation of a common data plane for shuffle libraries, i.e. the distributed futures backend.
The data plane must deliver the same performance and reliability as a monolithic shuffle system.
This is challenging because of the granularity of system operations: unlike a specialized shuffle system, which has a notion of a map and a reduce stage and can optimize transfer of intermediate blocks accordingly, a distributed futures system is not specific to shuffle and must treat each task and object as an independent unit.
Indeed, while Dask offers a distributed futures-based shuffle, its developers actually recommend using a custom shuffle implementation that bypasses their distributed futures backend because of scheduler scalability limits~\cite{dask-better-shuffling}.


Next, we identify the components of a distributed futures system that are necessary for performance and reliability of shuffle-as-a-library.
First, to coordinate the shuffle between mappers and reducers, we use a shared-memory distributed object store that acts as an intermediary: map tasks store their outputs in the object store and reduce tasks retrieve their arguments from the object store. \ion{How else could you use the shared object store?}
Second, for efficiency, the system transparently overlaps task execution with block I/O across the shared-memory object store, local disk, and network.
Third, the system implements timely garbage collection to ensure memory availability and reduce write amplification.
Finally, for fault tolerance, the system uses lineage reconstruction to ensure that each object required by the shuffle library is still reachable in the presence of failures.


Thus, we present \sys, a flexible shuffle system.
We build \sys on Ray, a distributed futures system for Python~\cite{ray,ownership}.
To meet the demands of large-scale shuffle, we extend Ray to support high-throughput spilling to disk and pipelining between block I/O and execution~(\cref{sec:arch}).
We show that the \sys implementations of previous shuffle strategies match the performance characteristics of their monolithic counterparts.
We also run a 100\,TB TeraSort benchmark on a cluster of 100 HDD nodes and find that \sys outperforms Spark by $1.8\times$.
Finally, we show that \sys can easily integrate with applications such as distributed ML training, improving end-to-end training throughput by $2.4\times$.
To summarize, our contributions are:
\begin{itemize}
    \item Demonstrate how distributed futures can be used to rewrite a variety of monolithic shuffle optimizations as application-level libraries, with an order of magnitude less code.
    \item Design and implement a distributed futures backend that scales shuffle-as-a-library to 100\,TB or more, matching or exceeding the performance of monolithic shuffle systems.
    \item Implement a broad set of applications on top of our backend to easily take advantage of previous shuffle work.
\end{itemize}









==> intro.tex <==
\section{Introduction}

The distributed futures interface is an extension to RPC that combines futures and distributed memory.
It allows applications to express distributed computation without having to specify when and where to schedule task execution and to move data.
It is especially useful because it promotes interoperability between data-intensive applications.
\swang{We need more of an intro (and citations) for distributed futures. Specifically, we need to: (1) define them more clearly, ideally with an example, (2) make the argument that such an abstraction is inevitable. We can pull directly from the HotOS and ownership papers for these; the hard part will be getting it concise.}

In designing abstractions for distributed programming, there are three main aspects to consider: (a) how general-purpose the abstractions are; (b) how powerful the features provided by the system are, and (c) how much performance can the applications achieve.
Distributed futures score highly in (a) by providing low-level programming primitives such as functions and objects, and also in (b) by providing powerful system features such as scheduling, distributed memory management and fault tolerance. However this makes it more difficult to achieve high performance (c) with distributed futures, because the execution system has less awareness of the application semantics.
\lsf{Should we first put out the a/b/c requirements we want for a distributed programming abstraction, and delay the introduction of distributed futures?}
\samyu{I think so; it would flow better from "three main aspects" to "application where providing all three aspects is hard"}

One example of an application that often requires specialized optimizations is distributed shuffle. It is a difficult task because it involves many aspects of the system: CPU, memory, networking and disk I/O, and that achieving high performance requires I/O efficiency and pipelining to saturate all parts of the system. \samyu{I think a lot of applications do involve these elements of the system, but with shuffle what's hard (from my understanding) is that there's (1) many-to-many communication that (2) requires large data movement regardless of locality policies.} \swang{+1 to Samyu's comment. We should start from the all-to-all communication part, then explain why that requires I/O efficiency, etc.} As such, people often build specialized distributed systems for shuffle to address performance concerns. For example, Spark built an external shuffle service~\cite{spark_ess} for improved reliability, and later integrated Magnet~\cite{magnet}, which implements new optimizations such as push-based shuffle to further solve scalability challenges.\cite{magnet,riffle,cosco,uberrss,alibaba_emr}

These dedicated shuffle systems achieve high performance (c) and provides powerful features (b), but are not general-purpose for distributed programming.
This makes it difficult to develop new algorithms. As an example, implementing push-based shuffle in Spark requires building a new system, which took TODO years to integrate into Spark~\cite{TODO}.
Furthermore, specialized systems make interoperability with other distributed applications hard. For example, it would not be possible to pipeline a machine learning training program with a shuffle operation using such systems without waiting for the full shuffle operation to complete. \samyu{Maybe reference one image in the diagram Stephanie suggested with visual representations of pipelining under different shuffles, except this is high level -- shuffle service w/ other app services?} \swang{+1 to adding a figure!}
\ekl{yep I think we need to have two figures in the intro: one for pipelining dag, and one showing the normal/magnet/riffle dags, and their distributed futures version. This is to emphasize how they can be "ported" to distributed futures}

In this paper we pose the question: what is required to achieve high performance for specialized applications like shuffle using a general-purpose distributed programming abstraction?
If we can implement shuffle efficiently on a general-purpose distributed system, then we can enable interoperability with other data-intensive applications, and faster development of new shuffle optimizations.

The answer: we use distributed futures~\cite{hotos-rpc} as an application-level programming abstraction for managing shuffle blocks, and run the application on a general-purpose distributed execution system, which manages task execution and distributed memory.
\lsf{We could delay the introduction of distributed futures until here.} \samyu{+1; also, maybe define task, since Ray has a fairly specific notion of what that is?} \swang{That's a possibility but we do want to make sure there is a clear idea of what we're proposing by this point, which could be difficult if we delay the introduction. That said, I do think it would be more streamlined if we go with Ion's proposal at the end of this intro (making the comparison RPC vs distributed futures instead of distributed futures vs external shuffle services). Also, this paragraph could better delineate what has been done before in existing systems for distributed futures vs. what this paper is proposing.}

At the system level, we implement general optimizations that will benefit any kind of workload, without specializing the system for shuffle operations.
We demonstrate that we can achieve all of the same optimizations as those implemented in specialized shuffle systems, which are categorized by the following three challenges.

\lsf{Need to introduce basic shuffle terminology so readers don't get lost in the details.}

First, I/O efficiency is a common challenge to large-scale shuffle. Assuming the partition size is fixed, the number of intermediate shuffle blocks grows quadratically with the total data size, while the size of the blocks decreases linearly. This leads to too many blocks of too-small sizes that the system needs to handle, which could lead to degraded networking and disk I/O efficiency.
A common solution is by merging the shuffle blocks at either the map or reduce side to reduce the total number of blocks, and also increase the block sizes~\cite{cosco,magnet,TODO}.
We implement the merging of shuffle blocks at the application level.
The system handles object transfer over the network, as well as spilling to and restoring from disk.
\lsf{Do we do any gRPC tricks for network transfer? Is fusing objects during disk spilling relevant here?}
Since the system only spills objects when memory is low, it is also important to have precise memory management through reference counting, in order to avoid unnecessary spilling, which would compete for disk bandwidth.

Second, achieving high performance requires pipelining disk, network and CPU operations.
Traditional shuffle is usually pull-based, in which reduce tasks only pull the shuffle blocks from the map tasks when they are scheduled to execute.
In addition to the small blocks problem, this also does not pipeline network transfer with disk operations.
Push-based shuffle~\cite{NADSort,magnet,TODO} solves this problem, where map tasks directly push the blocks onto the reducer side. This improves network utilization, and combined with merging blocks on the receiving end, also improves disk I/O efficiency.
To implement push-based shuffle at the application level without asking the system for a ``push'' functionality, we schedule map tasks and ``merge'' tasks in waves. Since the system pre-fetches arguments for a task prior to its execution, this effectively acts as push-based shuffle.

Third, fault tolerance is important for the reliability of large-scale shuffle operations.
One major benefit of external shuffle services~\cite{TODO} is that it decouples the lifetime of shuffle blocks from map task executors, so that the shuffle operation can endure executor failures without having to re-execute map tasks.
This is achieved in our system design: shuffle blocks are stored in the distributed object store, which is in a process separate from worker processes.
TODO: moving vs copying shuffle blocks, a tuning knob for fault tolerance. System implements generic per-task re-execution.

Evaluation: we run the Terasort benchmark.
Small working set, we are TODO\% faster than Magnet (thanks to our in memory object store).
Large data size up to 100TB, we are TODO\% faster than Spark native and Magnet.
We also run a data processing + shuffle + ML pipeline. Latency to GPU is TODO\% faster than baseline using Spark. End-to-end we are TODO\% faster.

Our contributions:
\begin{itemize}
\item We show that shuffle can be implemented on a general-purpose distributed programming interface such as distributed futures.
We identify and implement several features in the execution system to support shuffle, including object spilling, and moving of primary object locations.
\item We demonstrate that such implementation can reach TODO\% of the theoretical performance, and that it can outperform dedicated shuffle services on the TeraSort benchmark by TODO\%.
\item We implement shuffle in a distributed machine learning application, and show that the data latency can be reduced by TODO\%, and end-to-end latency reduced by TODO\%, when compared with a strawman solution that performs shuffle using a separate system.
\end{itemize}

\lsf{Ion's comments: Need to be more precise about distributed futures as ``a general-purpose distributed programming interface''. RPC is already one. One way to rewrite:\begin{itemize}
    \item Shuffle is an important primitive in data processing applications.
    \item Typically shuffle is implemented using low-level primitives like RPC. This makes it complicated because it leaves everything else manual: block memory management, network transfer, pipelining.
    \item In this paper we explore how we can implement shuffle using a higher-level abstraction. Ray offers distributed futures as a programming primitive. It is RPC + distributed memory management. It also handles scheduling, pipelining by prefetching task arguments, fault tolerance by retrying tasks, albeit all for generic tasks (without knowing application semantics). Benefits: this simplifies implementation (we can implement shuffle in X lines of Python), while preserving the flexibility to do performance optimizations and being able to achieve high performance; can interoperate with other data applications.
\end{itemize}
}

The rest of the paper is organized as follows. TODO





==> shuffle.tex <==
\section{Shuffle with Distributed Futures} \label{sec:shuffle}


\subsection{Distributed Futures}

We show that shuffle coordination, block management, and fault tolerance can be factored out into a common generic system for distributed memory management, much like RPC factors out remote task execution.
For this purpose, we use the \emph{distributed futures} API~\cite{ciel,ownership,hotos-rpc}, an extension of RPC that provides automatic memory management for a shared and immutable address space.

In this API, a program can invoke methods, known as \emph{tasks}, that execute and return data on a remote node.
When calling a remote function, instead of receiving the function's return value directly, the caller receives a distributed future that represents the \emph{eventual} return value.
In addition, the future is ``distributed'' because the return value may be stored anywhere in the cluster, e.g., at the node where the function executed.
This allows us to avoid copying RPC return values back to the caller, which can become a bottleneck for large data.

The caller can then resolve the value of the distributed future in two ways.
It can get the value of the distributed future using a \texttt{get} call, which fetches the value to the caller's local memory.
It can also pass the distributed future as an argument to another remote function.
In this case, the system ensures that the dependent task does not run until all of its arguments are computed and local to the executor.
Note that the caller can specify such dependencies before the value has been computed and that the caller never sees the physical values.
This gives the system control over parallelism and data movement, e.g., pipelining task execution with dependency fetching for other tasks, and allows the caller to manipulate data larger than local memory.

In the following sections, we show how to use these semantics to express many of the optimizations explored by previous shuffle systems in just a few lines of code.
For illustration purposes, we use the distributed futures API adopted by Ray~\cite{ray}, a popular distributed futures system for Python.
The \code{@ray.remote} annotation designates remote functions, and the \code{.remote()} operator invokes tasks.
\code{ray.get} fetches the return value of a function locally.
We also use \code{ray.wait} to wait for tasks to complete without having to fetch the return values locally.
Finally, we use the \code{del} operation in Python to delete distributed futures that we no longer need, indicating to the system that it is safe to garbage-collect the values.


\subsection{Shuffle at the Application Level} \label{sec:shuffle:impl}

We discuss the shuffle strategies used in previous monolithic systems~(\cref{fig:shuffle-dags}) and demonstrate how they can be implemented as application-level programs using Ray's distributed futures API.


\subsubsection{Simple Shuffle} \label{sec:shuffle:impl:naive}

\Cref{lst:simple-shuffle} shows a straightforward implementation of the MapReduce paradigm illustrated in \Cref{fig:shuffle-dags:naive}.

\begin{codeblock}{highlightlines=11-12}{listings/shuffle-simple.py}
\caption{``Simple'' shuffle.}
\label{lst:simple-shuffle}
\end{codeblock}

The code in \Cref{lst:simple-shuffle} assumes a few pre-defined constants and functions:
\begin{itemize}
    \item \code{M}, denoting the number of map tasks;
    \item \code{R}, denoting the number of reduce tasks;
    \item \code{load_partition}, a function that takes a partition ID and loads a data partition from a data source, such as AWS S3. Locality constraints can be specified with the task's resource requirements.
    % \code{.options(resources={"node:<ip>": 1})}~(\cref{sec:arch:objstore});
    \item \code{sort_and_partition}, a function that sorts the data and returns a list of indices $\{(s_i, e_i)\}_1^R$ such that \code{data}$_{s_i:e_i}$ should be sent to reducer $i$;
    \item \code{merge_sorted}, a function that merges many sorted blocks in the same data range into one output partition.
\end{itemize}

The two highlighted lines produce the task graph shown in \Cref{fig:shuffle-dags:naive}. Note that the \code{.remote()} calls are non-blocking, so the entire task graph can be submitted to the system without waiting for any one task to complete.


This is effectively \emph{pull-based shuffle}, in which shuffle blocks are \emph{pulled} from the map workers as reduce tasks progress.
Assuming a fixed partition size, the total number of shuffle blocks will grow quadratically with the total data size~(\cref{fig:shuffle-dags:naive}).
Thus, this strategy is well known to suffer from the problem of I/O efficiency and per-block metadata overhead.
\Cref{sec:eval:compare} shows empirical evidence of this problem: as the number of shuffle blocks increases, the performance of the naive shuffle implementation drops due to decreased I/O efficiency.
Prior works~\cite{riffle,magnet,cosco} have proposed solutions to this problem, which we study and compare next.


\subsubsection{Pre-shuffle Merge} \label{sec:shuffle:impl:riffle}

Riffle~\cite{riffle} is a specialized shuffle system built for Spark. Its key optimization is merging small map output blocks into larger blocks, thereby converting small, random disk I/O into large, sequential I/O before shuffling over the network to the reducers.
The merging factor $F$ is either pre-configured, or dynamically decided based on a block size threshold.
During execution, as soon as $F$ map tasks finish on an executor node, their output blocks ($F\times R$) are merged into $R$ blocks, each consisting of $F$ blocks of data from the map tasks.
This strategy, illustrated in \Cref{fig:shuffle-dags:riffle}, is shown as a distributed futures program in \Cref{lst:two-stage-shuffle} (\code{shuffle_riffle}).
The code additionally assumes \code{F} to be the pre-defined merge factor.

\begin{codeblock}{highlightlines={7-8,15-16}}{listings/shuffle-two-stage.py}
\caption{Riffle- and Magnet-style shuffle implementations.}
\label{lst:two-stage-shuffle}
\end{codeblock}

Riffle's key design choice is to merge map blocks locally before they are pulled by the reducers, 
as shown in the highlighted lines.
The merge function reduces an $F \times R$ array of blocks into $F$ merged blocks.
For simplicity, the code assumes that the first $F$ map tasks are scheduled on the first worker, the next $F$ map tasks on the second worker, etc.
In reality, the locality can be determined using scheduling placement hints and/or runtime introspection (\cref{sec:arch:objstore:refs}).
\Cref{sec:eval:compare} shows that this implementation of Riffle-style shuffle improves the job completion time over simple shuffle.


\subsubsection{Push-based Shuffle} \label{sec:shuffle:impl:magnet}

Push-based shuffle~(\cref{fig:shuffle-dags:magnet}) is an optimization that pushes shuffle blocks to reducer nodes as soon as they are computed, rather than pulling blocks to the reducer when they are required.
Magnet~\cite{magnet} is a specialized shuffle service for Spark that performs this optimization by merging intermediate blocks on the reducer node before the final reduce stage.
This improves I/O efficiency and locality for the final reduce tasks.
\code{shuffle_magnet} in \Cref{lst:two-stage-shuffle} implements this design.





\subsection{Pipelining} \label{sec:shuffle:pipelining}

The key to achieving high-performance shuffle is ensuring high utilization of all system components: CPU, memory, disk and network.
We can do this by pipelining the tasks such that when one part of the system is busy (e.g. CPU is sorting and data is in memory), another part of the system works on another round of tasks (e.g. writing output to disk).
While the distributed futures system implements some pipelining~(\cref{sec:arch:memory}), the application can also give hints to the system by limiting which tasks are allowed to execute concurrently.

In \sys, the intra-shuffle pipelining shown in \Cref{fig:shuffle-dags:pipeline} can be expressed at the application level by scheduling tasks in rounds, as shown in \Cref{lst:pipelining}.

\begin{codeblock}{}{listings/pipelining.py}
\caption{Pipelined scheduling of map and merge tasks.}
\label{lst:pipelining}
\end{codeblock}

The code skeleton in \Cref{lst:pipelining} works for both the Riffle- and Magnet-style shuffle algorithms in \Cref{lst:two-stage-shuffle}.
Map and merge tasks are scheduled in \emph{rounds} according to the task parallelism \code{P}. At round $i$, the application will:
\begin{enumerate}
    \item Submit the $i$-th round of map tasks.
    \item Block until the last round of merge tasks finish.
    \item Submit $i$-th round of merge tasks to consume the $i$-th round of map tasks' outputs.
    \item Delete the $i$-th round of map tasks' outputs.
\end{enumerate}

The first three steps ensure that there is at most one round of merge tasks and one round of map tasks that can execute concurrently.
Because merge tasks consume the outputs of map tasks, this ensures that the producers will not outpace the consumers.

The fourth step acts as a hint to the system that the map outputs can be garbage-collected as soon as their consumers (the merge tasks) complete.
This also shows how \sys can be used to reduce \emph{write amplification}, similar to the system Cosco.
Cosco~\cite{cosco} is a shuffle service designed for disaggregated storage architecture that uses an intermediate merge similar to \Cref{fig:shuffle-dags:magnet}.
Besides the difference in block storage, Cosco also features the reduction of write amplification---in Riffle and Magnet, each map output block is written to disk once when it is created, then once more when it is merged, and one more time in the reducer output, causing a $3\times$ write amplification~\cite{cosco}.
Cosco reduces the write amplification factor to $2\times$ by creating the shuffle blocks in memory and only spilling the merge outputs to disk.

In \sys, the application achieves this by choosing \code{P} such that the outputs produced by \code{P} concurrent map tasks will not exceed in-memory object store capacity.
In combination with timely garbage collection~(\cref{sec:arch:objstore:refs}), this avoids the initial write to disk when a map output block is created.
The tradeoff is that since the system deletes all copies of the intermediate map outputs, we will also need to re-execute all previous map tasks in case of a failure.
In contrast, the Riffle- and Magnet-style~(\cref{lst:two-stage-shuffle}) programs both keep all distributed futures in scope, meaning that the system will keep copies of all the intermediate blocks.
This can be expressed at the application level by replacing step 4 with a line that keeps all map outputs in scope, e.g., \code{all_map_outs.append(map_out)}.


\subsection{Fault Tolerance} \label{sec:shuffle:ft}

Failures in distributed systems happen for a multitude of reasons, including network failures, machine failures and process restarts. In shuffle, network failures can prevent workers from sending or fetching shuffle blocks. Machine failures and process restarts can further result in data loss and require in-progress tasks to be re-executed.

In \Cref{sec:arch:ft}, we discuss how the distributed futures system can tolerate and transparently recover from these failures on behalf of the application.
The main requirement from the application is that each remote function defined by the application is idempotent and side-effect-free.
Also, note that while the task graph is generated dynamically, the arguments to each individual task are immutable, as the distributed futures that the task depends on must be specified at invocation time.
This prevents consistency problems in cases where the system must retry a task or object transfer.






\subsection{Straggler Mitigation} \label{sec:shuffle:straggler}

Stragglers are tasks that take longer to finish than most other tasks. If not properly handled, they significantly delay the job completion time.
Data skew is a related problem, where data is unevenly distributed, causing some reduce tasks to receive more work than others and become stragglers.
\Cref{appx:sec:stragglers} presents two application-level strategies for straggler mitigation, namely speculative execution and best-effort merge.


\subsection{Application Interoperability} \label{sec:shuffle:app}

A major benefit of \sys is that since shuffle is implemented at the application level, it can easily interoperate with other non-shuffle applications.
In this section, we demonstrate two example applications in which fine-grained pipelining of shuffle with other applications~(\cref{fig:shuffle-dags:pipeline}) can improve end-to-end job performance.

\subsubsection{Online Aggregation: Streaming Shuffle}

Online aggregation~\cite{online-aggregation} is an interactive query processing mode where partial results are returned to the user as soon as some data is processed, and are refined as progress continues.
While a useful interaction mode, it is non-trivial to implement in MapReduce systems due to their batch processing nature.
Past work made in-depth modifications to Hadoop MapReduce and Spark to support online aggregation~\cite{mapreduceonline, g-ola}.

Online aggregation is straightforward to implement in \sys because it does not require modifying the underlying distributed futures system.
\Cref{lst:online-aggregation} shows an example of a word count program modified for online aggregation.
The driver fetches reduce results as they become available, enabling the program to produce a top-K estimate as soon as the first reduce tasks finish.


\begin{codeblock}{}{listings/online-aggregation.py}
\caption{Shuffle pipelined with online aggregation.}
\label{lst:online-aggregation}
\end{codeblock}


\subsubsection{Shuffling Data Loader for Distributed Machine Learning Training}

In distributed machine learning training, training data is partitioned and stored on each training node.
At every epoch, training data is randomly shuffled across all nodes before it is loaded into distributed GPUs.
Shuffling the training data is important for de-correlating training samples, preventing overfitting, and improving convergence~\cite{randomreshuffling}.
This is straightforward to implement using distributed futures, as shown in \Cref{lst:shuffle-ml}.
Note that we use Ray \emph{actors}, or stateful workers, to hold the state for each model replica.

\begin{codeblock}{}{listings/shuffle-ml.py}
\caption{Shuffling data loader for distributed machine learning training.}
\label{lst:shuffle-ml}
\end{codeblock}

By pipelining reducer outputs from the \code{shuffle} routines shown in \Cref{lst:simple-shuffle,lst:two-stage-shuffle} directly into the machine learning trainers, model training can start as soon as the first batch of data arrives, and data can be transferred entirely in-memory.
Furthermore, tasks in the \code{shuffle} routine can be pipelined with the \code{Trainer.train} tasks.
This is again non-trivial to achieve in traditional batch processing systems such as Spark, which  provides only \emph{synchronous} semantics for shuffle and high-level APIs for dataset manipulation~(\cref{fig:shuffling-data-loader-ml}).
We evaluate the benefits of this fine-grained pipelining in \Cref{sec:eval:app} and show that the latency to the first batch of results can be reduced by 70\%.

\begin{figure}[ht!]
  \centering
  \includegraphics[width=\linewidth]{figures/ml-pipeline}
  \caption{Shuffle pipelined with distributed ML training.}
  \label{fig:shuffling-data-loader-ml}
\end{figure}

